PromptAid: Prompt Exploration, Perturbation, Testing and Iteration using Visual Analytics for Large Language Models

Large Language Models (LLMs) have gained widespread popularity due to their ability to perform ad-hoc Natural Language Processing (NLP) tasks with a simple natural language prompt. Part of the appeal for LLMs is their approachability to the general public, including individuals with no prior technical experience in NLP techniques. However, natural language prompts can vary significantly in terms of their linguistic structure, context, and other semantics. Modifying one or more of these aspects can result in significant differences in task performance. Non-expert users may find it challenging to identify the changes needed to improve a prompt, especially when they lack domain-specific knowledge and lack appropriate feedback. To address this challenge, we present PromptAid, a visual analytics system designed to interactively create, refine, and test prompts through exploration, perturbation, testing, and iteration. PromptAid uses multiple, coordinated visualizations which allow users to improve prompts by using the three strategies: keyword perturbations, paraphrasing perturbations, and obtaining the best set of in-context few-shot examples. PromptAid was designed through an iterative prototyping process involving NLP experts and was evaluated through quantitative and qualitative assessments for LLMs. Our findings indicate that PromptAid helps users to iterate over prompt template alterations with less cognitive overhead, generate diverse prompts with help of recommendations, and analyze the performance of the generated prompts while surpassing existing state-of-the-art prompting interfaces in performance.

==> 03_background.tex <==
\vspace{-2mm}
\section{Background on Reinforcement Learning}
\label{sec:background}

% Reinforcement learning is a technique in which the 
% Reinforcement learning is a branch of AI where an \textit{agent} \textit{interacts} by a set of \textit{actions} with the \textit{environment} which are represented by a set of \textit{states} to gain a certain \textit{reward}. \hl{Make agent env diagram}.

% The major difference between Reinforcement Learning and Machine Learning is that in RL the learning process involves interaction between the agent and it's environment without the need of an external agent to teach anything to the RL agent. 
% The major aim of the reinforcement learning agent is to maximize it's rewards over time. The agent explores and exploits the environment iteratively till it achieves an understanding of the environment. The output of such a training process is a \textit{policy}. A policy is a state to action mapping for the agent in a particular environment. An optimal policy is the one which helps the agent maximize it's rewards over time. 

Reinforcement learning is a technique to train an autonomous \textbf{agent}, in which the agent interacts with the environment and learns to achieve some desired \textbf{goal} through trial-and-error. In contrast to supervised learning, the agent does not require a training set of labeled examples for the desired behavior; likewise, RL differs from unsupervised learning by not simply learning patterns from unlabeled data. Rather, the agent learns the desired behavior using its own experience interacting with the environment. An agent's overall goal can be defined in terms of a special signal called a \textbf{reward} that the agent gets for taking some action in the environment. Informally, the agent is tasked with learning a behavior that would maximize the total amount of reward it receives in the long term. Concretely, the problem of reinforcement learning can be formalized in terms of a \textbf{Markov decision process} (MDP).

\subsection{Markov Decision Process}
\label{sec:mdp}
% Markov decision process (MDP) is the all at the crux of a Reinforcement learning paradigm. The RL agent's underlying MDP \( \mathbb{M} \) is defined by a tuple $\langle S,A,R,T,\gamma \rangle$ where \textit{S} is a set of all possible atomic states, \textit{A} represents a set of possible actions, \textit{T} is the transition function, \textit{R} is the reward and $\gamma$ is the discounting factor where, $0 \leq \gamma\ < 1$. $T : S \times A \times S \rightarrow [0,1]$ is the probability that given a state \textit{s} and taking an action \textit{a} would lead to a new state \textit{s'} and $R : S \times A \times S \rightarrow \mathbb{R}$ is the reward corresponding to the transition. The solution on solving a MDP \( \mathit{M} \) is a policy $\pi$. A policy is an optimal one when the expected future rewards from all states is maximum. A trajectory denoted as $(\langle s_1,a_1,s_2 \rangle, \langle s_2,a_2,s_3 \rangle, .... \langle s_{n-1},a_{n-1},s_{n} \rangle)$ however is a path that the agent takes from the start state till the goal is achieved. The actions taken in each of those states is determined by the policy. 


% \textbf{Maximizing and calculating future rewards - }The total reward an agent achieves on completion of one episode would be $R = r_1 + r_2 + ... + r_n$ where n is the number of steps it took the agent to finish one episode. However the problem with such a calculation of reward is that the agent might take an infinite amount of time to finish the task thus leading to an infinite reward. Thus the discount factor helps the algorithm to converge. Thus the reward is then calculated as - $R = r_1 + \gamma r_2 + \gamma^2 r_3 + .... + \gamma ^n r_n$. Thus the reward at any time is the reward achieved till that time plus the discounted future rewards. This can be calculated using the bellman equation. The bellman equation is given by - 
% \begin{equation}
% Q(s,a) = \sum_{s'} T(s,a,s')[R(s,a,s') + \gamma max_{a}Q(s,a)]
% \end{equation}
% Thus to maximize future rewards this equation can be solved using dynamic programming. 

MDP formulates a sequential decision-making task where, at each time step, the agent observes the current \textbf{state} of the environment and decides to take an \textbf{action}. This transitions the environment to its next state and the agent receives a reward. The agent keeps acting in the environment until it reaches a terminal state at some time step $T$. The reward the agent obtains for each step is discounted with a discount factor $\gamma$. The total reward obtained by the agent for the sequence of transitions is subsequently defined as the \textbf{return}, $G = \sum_{t=1}^{T}\gamma^{t-1}R_{t}$ where $R_{t}$ is the reward obtained for the $t^{\text{th}}$ transition.

Formally, a MDP is defined as a tuple $\langle \mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \gamma \rangle$ where $\mathcal{S}$ is the set of all possible states of the environment, $\mathcal{A}$ is the set of all possible actions the agent can take at any state, $\mathcal{T} \colon \mathcal{S} \times \mathcal{A} \times \mathcal{S} \to [0, 1]$ is the transition function where $\mathcal{T}(s, a, s')$ gives the probability that the environment will transition to a state $s'$ when the agent takes an action $a$ in state $s$, $\mathcal{R} \colon \mathcal{S} \times \mathcal{A} \times \mathcal{S} \to \mathbb{R}$ is the reward function that gives the reward the agent obtains when it takes an action $a$ in state $s$ causing a transition to state $s'$, and $\gamma$ is the discounting factor applied to the obtained rewards. 

Given an MDP, a \textbf{policy} $\pi$ maps each state to some action $a \in \mathcal{A}$. The \textbf{value} for any state is then the expected return the agent gets when it follows the policy $\pi$ starting from the state. The goal of the agent is to learn a policy, referred to as the \textbf{optimal policy} $\pi^{*}$, that maximizes the value for each state. Lastly, the $Q$-value function, $Q_{\pi}(s, a)$ gives the value obtained obtained if the agent takes the action $a$ in state $s$ and then follow the policy $\pi$. If all the components of the MDP are known to the agent, then it can learn $\pi^{*}$ as $\pi^{*}(s) = \argmax_a Q^{*}(s, a)$, where the $Q^{*}(s, a)$ is obtained by solving the following Bellman optimality equation using dynamic programming algorithms like value iteration or policy iteration\cite{sutton2018reinforcement} : $Q^{*}(s,a) = \sum_{s'} \mathcal{T}(s,a,s')[\mathcal{R}(s,a,s') + \gamma .max_{a}Q^{*}(s',a)]$

% \begin{equation*}
% 	Q^{*}(s,a) = \sum_{s'} \mathcal{T}(s,a,s')[\mathcal{R}(s,a,s') + \gamma .max_{a}Q^{*}(s',a)]
% \end{equation*}

\subsection{Interpreting State Features}
\label{sec:interpresting_features}

In this work, we assume each state $s$ of the environment can be expressed as a feature vector $\langle f_1, f_2, \dots, f_n\rangle$ where each feature $f_i$ can be understood by the domain expert that will be using \name{} (this is in line with the policy explanation technique presented in~\cite{hayes2017improving}, where states can be described in terms of binary features via classifiers). For example, for the HIV drug recommendation domain, states are defined via features like \textsf{the number of infected lymphocytes}, \textsf{immune response}, etc. \name{} provides explanations in terms of these features. For simplicity, we pick domains where the states were already defined in terms of features that a human can understand. Hence, the state features that the agent views during interaction with the environment would be the same as the one used for explanations. However, this is not a requirement for our system to work. See Section~\ref{sec:discussion} for discussion about relaxing this requirement in future work.

\subsection{Model-Based and Model-Free Learning}
% These two methods are the two different branches in RL. Model based RL methods involves the usage of transition dynamics which is used to find optimal actions for the agent. This method works perfectly well when the transitions and rewards can be stored and aren't huge in number. However many of the real world applications or even games as simple as pacman involve millions of states and finding the transition dynamics for each state would be a time consuming process. 

% Some pros and cons of each of the technique are - (1) Model based RL agents reach an optimal solution faster and are also quite sample efficient. The latter means using less amount of data to make a decision. However a model free RL agent is more error prone which leads us to the advantages of model free RL methods. (2) Model free RL methods are very easy to implement and does not need the agent to know the state dynamics beforehand. 

RL algorithms can be classified as either \textbf{model-based} and \textbf{model-free}~\cite{sutton2018reinforcement}. In model-based RL, the agent learns the model of the environment (specifically, it learns the model components of the MDP incorporating the environment dynamics) and uses that to derive the optimal policy. Conversely, model-free RL algorithms do not require a learned model to obtain the optimal policy.

In this work, we use algorithms from both the classes to train our agent for different domains. For the model-based approach, we assume access to the state set $\mathcal{S}$, and employ a simple sampling strategy to learn the model parameters $\mathcal{T}$ and $\mathcal{R}$. With this strategy, for each state $s \in S$, each action $a \in A$ is executed $k$ times. The value of $\mathcal{T}(s,a,s')$ is then set to $k'/k$ where $k'$ is the number of times the environment transitions to state $s'$ when the agent took the action $a$ in state $s$. The value of $\mathcal{R}(s,a,s')$ is set as the average reward obtained for the transitions $\langle s, a, s'\rangle$. Once the model is learned, we compute the optimal policy using policy iteration.

For the model-free approaches, we use function approximation based methods that learn the Q-function directly from agent's experience. The learning involves the agent interacting with the environment over several episodes improving its Q-function estimate. In each episode, the agent starts at some random initial state and follows an $\epsilon$-greedy policy in which the agent chooses an action that maximizes its $Q$ value with a probability of $1-\epsilon$ or chooses to do a random action (uniformly sampled) with probability $\epsilon$.  
% \vspace{-4.5mm}
% \begin{equation*}
%     \pi(s)=\begin{cases}
%           \argmax_a Q(s,a) \quad &\text{with probability} \, 1 - \epsilon \\
%           \text{uniform random action} \quad &\text{with probability} \, \epsilon \\
%      \end{cases}
% \end{equation*}
The agent collects experience using the $\epsilon$-greedy policy and then uses it to approximate the $Q$-function. For our domains, we used linear function and neural network based approximations. The former technique represents the $Q$-function as a weighted linear function of features $f_i$ defined over the state:
$
    Q_{\theta}(s, a) = \theta_{1}.f_{1}(s) + \theta_{2}.f_{2}(s) + \dots + \theta_{n}.f_{n}(s)
$
The weights are updated after each individual interaction with the environment, where the agent takes an action $a$ in state $s$ resulting in it transitioning to state $s'$ getting a reward $r$, using the following update equation where $\alpha$ is the learning rate:
$
    \theta_{i} = \theta_{i} + \alpha * [r + \gamma.max_{a}Q_{\theta}(s', a') - Q_{\theta}(s, a)]f_{i}(s)
$

For the neural network based $Q$-function approximation, we trained a fully connected neural network using the same strategy as the one used to train deep Q-networks (DQN) in \cite{mnih2013playing}. The neural network given by $Q(s, a, \theta)$, where $\theta$ represents the weights of the network, approximates the $Q$-value function corresponding to the optimal policy i.e. $Q^{*}(s, a)$. The agent's transition at each time step, $\langle s, a, r, s' \rangle$ is stored in a database $D$. The database is of a fixed length and stores the most recent transitions. After each action is executed (which is treated as an iteration $i$ of the training algorithm), the Q-network is trained by optimizing the following loss function over a mini batch of transitions sampled uniformly from $D$: 
$
	L_{i}(\theta_{i}) = E_{(s,a,r,s') \sim D} [(r + \gamma max_{a'} Q(s',a'; \theta_{i-1}) - Q(s, a; \theta_{i}))^2].
$

In \name{} the Taxi Domain was trained using Model Based RL, StackBot using Approximate Q-learning and the HIV Domain using a DQN. 


==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

